Sparse Auxiliary Networks for Unified Monocular Depth Prediction and Completion

Estimating scene geometry from data obtained with cost-effective sensors is key for robots and self-driving cars. In this paper, we study the problem of predicting dense depth from a single RGB image (monodepth) with optional sparse measurements from low-cost active depth sensors. We introduce Sparse Auxiliary Networks (SANs), a new module enabling monodepth networks to perform both the tasks of depth prediction and completion, depending on whether only RGB images or also sparse point clouds are available at inference time. First, we decouple the image and depth map encoding stages using sparse convolutions to process only the valid depth map pixels. Second, we inject this information, when available, into the skip connections of the depth prediction network, augmenting its features. Through extensive experimental analysis on one indoor (NYUv2) and two outdoor (KITTI and DDAD) benchmarks, we demonstrate that our proposed SAN architecture is able to simultaneously learn both tasks, while achieving a new state of the art in depth prediction by a significant margin.

==> figures/figure_residual.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.32\textwidth]{images/residual.pdf}
\caption{\textbf{Sparse residual block} (SRB) used to process input depth maps. Each \textit{SparseConv2D} layer is a Minkowski 2D Convolution \cite{minkowski}, \textit{BN} is Batch Normalization \cite{bnorm} and \textit{ReLU} are Rectified Linear Units~\cite{relu}.}
\label{fig:residual}
\end{figure}


==> images/ZZZ/authors.tex <==
\author{
Vitor Guizilini \qquad Rare\cb{s} Ambru\cb{s} \qquad Wolfram Burgard \qquad Adrien Gaidon \\ % <-this % stops a space
Toyota Research Institute (TRI), Los Altos, CA \\
\texttt{\{first.lastname\}@tri.global}
%\thanks{*This work was not supported by any organization}% <-this % stops a space
%\thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
%        University of Twente, 7500 AE Enschede, The Netherlands
%        {\tt\small albert.author@papercept.net}}%
%\thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
%        Dayton, OH 45435, USA
%        {\tt\small b.d.researcher@ieee.org}}%
}
